Ptolemy: Architecture Support for Robust Deep Learning

Deep learning is vulnerable to adversarial attacks, where carefully-crafted input perturbations could mislead a well-trained Deep Neural Network to produce incorrect results. Today's countermeasures to adversarial attacks either do not have capability to detect adversarial samples at inference time, or introduce prohibitively high overhead to be practical at inference time. We propose Ptolemy, an algorithm-architecture co-designed system that detects adversarial attacks at inference time with low overhead and high accuracy.We exploit the synergies between DNN inference and imperative program execution: an input to a DNN uniquely activates a set of neurons that contribute significantly to the inference output, analogous to the sequence of basic blocks exercised by an input in a conventional program. Critically, we observe that adversarial samples tend to activate distinctive paths from those of benign inputs. Leveraging this insight, we propose an adversarial sample detection framework, which uses canary paths generated from offline profiling to detect adversarial samples at runtime. The Ptolemy compiler along with the co-designed hardware enable efficient execution by exploiting the unique algorithmic characteristics. Extensive evaluations show that Ptolemy achieves higher or similar adversarial example detection accuracy than today's mechanisms with a much lower runtime (as low as 2%) overhead.

==> opt.tex <==
\section{Optimization}
\label{sec:opt}

\subsection{Algorithm Optimization}
From algorithm perspective, we provide two optimizations. 

\textbf{Hybrid Execution}
We apply two kinds of hybrid execution in the framework to balance detection accuracy and computation complexity: direction hybrid and layer hybrid. 

Direction hybrid refers to detecting same samples with both forward extraction method and backward extraction method. If the forward extraction pattern returns to an detection result below the confidence threshold, we can further use backward extraction method to re-generate the pattern and detect whether it is a adversarial example or not. The direction hybrid combination solves the problem of backward extraction methods usually has higher accuracy while with longer latency while forward extraction methods can be processed faster but with a lower accuracy.

Layer hybrid refers to using different methods for different layers in either forward extraction process or backward extraction process. Mixing different types of methods among different layers in one example can balance the latency and computation cost. As well provide more flexibility to users when desigining algorithms against different attacks. 


\textbf{Early Termination and Late Start}
We apply early termination in the pattern extraction process. We prove that the latter layers contribute more in detecting the adversarial examples. Thus, we provide early termination in backward extraction and late start in forward extraction to reduce latency and energy cost. The degree of early termination and late start are provided to users as part of the programming model. 


\subsection{Compiler Optimization}


\textbf{Neuron Level Pipeline}
A key observation we make in pattern extraction process is that there is no neuron level dependency, enabling the possibility of execute the pattern extraction among different neurons in a software pipeline way. 

\textbf{Layer Level Pipeline}
For the forward extraction methods, tradition execution model will start pattern extraction method after inference. However, there is no dependency between different layers. We apply layer level pipeline execution model. Whenever the layer finishes inference, the pattern extraction pattern for that layer starts.  

\subsection{Hardware Optimization}

\textbf{Super Scalar Execution and SIMD}


\textbf{Augemented Inference}

